Multi-threaded Sparse Matrix-Matrix Multiplication for Many-Core and GPU Architectures

Sparse Matrix-Matrix multiplication is a key kernel that has applications in several domains such as scientific computing and graph analysis. Several algorithms have been studied in the past for this foundational kernel. In this paper, we develop parallel algorithms for sparse matrix-matrix multiplication with a focus on performance portability across different high performance computing architectures. The performance of these algorithms depend on the data structures used in them. We compare different types of accumulators in these algorithms and demonstrate the performance difference between these data structures. Furthermore, we develop a meta-algorithm, kkSpGEMM, to choose the right algorithm and data structure based on the characteristics of the problem. We show performance comparisons on three architectures and demonstrate the need for the community to develop two phase sparse matrix-matrix multiplication implementations for efficient reuse of the data structures involved.

==> references.tex <==
[?1049h[?1h=[1;55r[?12;25h[?12l[?25h[27m[m[H[2J[?25l[55;1H"spgemm.bbl" 162L, 6960C[1;1H% Generated by IEEEtran.bst, version: 1.13 (2008/09/30)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{edwards2014kokkos}
H.~C. Edwards, C.~R. Trott, and D.~Sunderland, ``Kokkos: Enabling manycore
  performance portability through polymorphic memory access patterns,'' \emph{J
  Parallel Distrib Comp}, vol.~74, no.~12, pp. 3202--3216, 2014.

\bibitem{openmpgpus}
J.~Beyer and J.~Larkin, ``Targeting gpus with openmp 4.5 device directives,''
  in \emph{Proceedings of the GPU Technology Conference}, 2016.

\bibitem{gustavson1978two}
F.~G. Gustavson, ``Two fast algorithms for sparse matrices: Multiplication and
  permuted transposition,'' \emph{ACM Transactions on Mathematical Software
  (TOMS)}, vol.~4, no.~3, pp. 250--269, 1978.

\bibitem{patwary2015parallel}
M.~M.~A. Patwary, N.~R. Satish, N.~Sundaram, J.~Park, M.~J. Anderson, S.~G.
  Vadlamudi, D.~Das, S.~G. Pudov, V.~O. Pirogov, and P.~Dubey, ``Parallel
  efficient sparse matrix-matrix multiplication on multicore platforms,'' in
  \emph{High Performance Computing}.\hskip 1em plus 0.5em minus 0.4em\relax
  Springer, 2015, pp. 48--57.

\bibitem{intel2007intel}
Intel, ``Intel math kernel library,'' 2007.

\bibitem{demouth2012sparse}
J.~Demouth, ``Sparse matrix-matrix multiplication on the gpu,'' in
  \emph{Proceedings of the GPU Technology Conference}, 2012.

\bibitem{liu2014efficient}
W.~Liu and B.~Vinter, ``An efficient gpu general sparse matrix-matrix
  multiplication for irregular data,'' in \emph{Parallel and Distributed[1;1H[?12l[?25h[?25l[55;1HType  :quit<Enter>  to exit Vim[1;1H[?12l[?25h[?25l[?12l[?25h[?25l[?12l[?25h
[?25l[55;1H[1m-- INSERT --[m[55;13H[K[2;1Hbegin{thebibliography}{10}[2;27H[K[2;1H[?12l[?25h[?25l[3;54r[3;1H[L[1;55r[2;1H[K[3;1Hbegin{thebibliography}{10}
[?12l[?25h[?25l[55;1H[K[3;1H[?12l[?25h[?25l[55;1HType  :quit<Enter>  to exit Vim[3;1H[?12l[?25h[?25l[?12l[?25h
[?25l[55;1H[1m-- INSERT --[m[55;13H[K[4;1Hprovidecommand{\url}[1]{#1}[4;28H[K[4;1H[?12l[?25h[?25lwprovidecommand{\url}[1]{#1}
w[?12l[?25h[?25lwaprovidecommand{\url}[1]{#1}
wa[?12l[?25h[?25ladprovidecommand{\url}[1]{#1}
wad[?12l[?25h[?25ldaprovidecommand{\url}[1]{#1}
wada[?12l[?25h[55;1H[?1l>[?1049lVim: Caught deadly signal HUP
Vim: preserving files...
Vim: Finished.
[55;1H
